Coinductive Soundness of Corecursive Type Class Resolution

Horn clauses and first-order resolution are commonly used to implement type classes in Haskell. Several corecursive extensions to type class resolution have recently been proposed, with the goal of allowing (co)recursive dictionary construction where resolution does not termi- nate. This paper shows, for the first time, that corecursive type class resolution and its extensions are coinductively sound with respect to the greatest Herbrand models of logic programs and that they are induc- tively unsound with respect to the least Herbrand models. We establish incompleteness results for various fragments of the proof system.

==> response.tex <==
\newpage
\section{Response to Reviewer Comments}

 We would
like to thank all reviewers for their helpful comments,  their suggestions helped us to improve this paper.
The major improvement we have made in this version of the paper is inclusion of detailed discussion of various kinds of completeness results possible for the proof system we describe, and
analysis of their relation to the existing literature and their inter-connections.
This line of work was suggested by Reviewer 3. We addressed all comments by all the reviewers, as we will explain in detail below.

\subsection{Response to Review 1}

The reviewer provided detailed comments on formulations of several sentences in
our paper and noticed some typographical errors, \eg repeated words. We made the suggested changes
accordingly. 
%in
%several places and we reformulated the text in the other also due to the
%comments of other reviewers. We do not discus these comments in a further detail.

The reviewer also suggested two further references. In the
first reference,

\vskip1em\noindent
Grigore Rosu and Dorel Lucanu. \emph{Circular coinduction --- a proof theoretical
foundation}. In CALCO 2009, volume 5728 of Lecture Notes in Computer
Science, pages 127--144. Springer, 2009.
\vskip1em

\noindent
the authors present a proof system for circular coinduction.  They state that
they do not prove soundness with respect to any model. Although we believe that
the reviewers suggestion on similarity of guardedness condition and freezing
operator is correct we do not believe that our paper is the right place to
discuss it since we are interested here in soundness with respect to Herbrand
models.

\newknote{Instead of alienating the reviewer by `` we do not believe that our paper is the right place to
discuss it'' -- just include the reference in related work, and explain the relation}

The other reference the reviewer provides is 

\vskip1em\noindent
Davide Sangiorgi. {\em An Introduction to Bisimulation and Coinduction}. Cambridge
University Press, 2012.
%A preliminary version of Chapter 2 from which
%we adapt paterial can be found at
%\url{http://www.cs.unibo.it/~sangio/DOC_public/corsoFL.pdf}.
\vskip1em

\noindent
We already cite one of Sangiorgi's earlier papers \cite{Sangiorgi09} and we
include this earlier reference where the reviewer suggests to include the above one 
since we believe it serves the purpose the reviewer intended.

\subsection{Response to Review 2}

The reviewer raised a question of novelty of material in the paper and its
overlap with Fu's \etal paper \cite{FuKSP16}. We changed the end of the
introduction of our paper to state more clearly that our paper studies soundness of the
calculus of extended corecursive type class resolution, which is not present in
Fu \etal, and also soundness of preexisting calculi. The novel contributions of our paper
are the theorems of coinductive soundness of the calculi in Section
\ref{sec:coind_sound} and Section \ref{sec:ext_coind_sound} and soundness of
program transformation methods. Also, in response to the comments the
reviewer 1 made, we include discussion of completeness, or lack thereof, in the
inductive and coinductive cases. We also consider this to be novel material.

We address the detailed comments the reviewer made as follows:
The reviewer noted that some explanation of why lambdas arise with the {\tt Bush}
example is appreciated. We include a reference that clarifies why such an
extension of resolution mechanism is necessary.

The reviewer noted that the sentence ``However, a lemma may overlap with other
axioms and lemmata'' was not clear. We clarified our definitions of an axiom and
a lemma in the context of axiom environment and we clarified the definition of
overlapping in the restrictions in the Section \ref{sec:intro}. 

Furthermore, the reviewer pointed out several formulations that were not clear
and some typographical errors. We clarified suggested parts of the text and we
fixed the typographical errors. %We do not discuss these in further detail.

\subsection{Response to Review 3}
The reviewer suggested there is a problem with the statement of the Theorem
\ref{thm:pt}. Indeed, a necessary condition that the proof term is in $\HNF$ was missing in the statement of the
theorem in the previously submitted version of the paper. We amended the
statement of the theorem and extended the explanation to make the use of this
condition clear.
\newknote{say what that condition is, otherwise it is cryptic}
\fnote{done}


Furthermore, the reviewer noted that we do not address the question of
completeness. He provided several conjectures of completeness results in
inductive and coinductive cases.
%We believe that the question of completeness is
%an interesting one and that his conjectures are in concordance with the future
%work we project in the Section \ref{sec:con}. However, we do not think that the
%page limit of the paper allows for proper analysis of the issue and we omit any
%partial analysis in favour of more thorough discussion of soundness results.
%
We now include a discussion of completeness both in inductive and coinductive cases in
the paper. It turned out that the question is not as simple as one might expect.
One can consider two different notions of completeness---first,
whether a ground atomic formula that is in $\MP$ has a proof in $\Phi_P$, and the other,
whether a formula (either an atomic formula or a Horn formula) that is valid in
$P$ has a proof in $\Phi_P$. The completeness results are as conjectured by the
reviewer for the first notion. But completeness fails in both inductive and
coinductive case in the other. We added this discussion into the paper.

We incorporated all minor remarks by the reviewer.

%also made some minor remarks. We incorporated these into the text
%and we do not discuss them further.






==> tex/complete.tex <==
\section{Completeness}



\begin{example}
The calculus of \ref{ir:lp-m} and \ref{ir:lam} is not complete in the inductive
case. Consider the following program with a function symbol $\mathtt{f}$:


\begin{alignat*}{3}
    \kappa_1 :~ & && \Rightarrow \mathtt{A}(\mathtt{f})\\
    \kappa_2 :~ & && \Rightarrow \mathtt{B}(\mathtt{f})\\
\end{alignat*}

\noindent
The least Herbrand model $\MP = \{A(f), B(f) \}$. Therefore 
$P \vDash_{ind} \mathtt{B}(x) => \mathtt{A}(x)$. 
However, any proof of $\mathtt{B}(x) => \mathtt{A}(x)$
needs to show that:

    \begin{prooftree}
        \footnotesize
        \AxiomC{\dots}
        \UnaryInfC{$
            (P, \alpha : ~\Rightarrow \mathtt{B}(x)) \vdash
            e : \mathtt{A}(x)$}
        \RightLabel{\sc Lam}
        \UnaryInfC{$
            P \vdash
            \lambda \alpha . e : \mathtt{B}(x) \Rightarrow \mathtt{A}(x)
        $}
    \end{prooftree}
\noindent
where $e$ is a proof term.
Since $\mathtt{A}(x)$ is not an implication and cannot proceed by the rule
\ref{ir:lam}. However, neither
$\mathtt{B}(x)$, nor any of heads of the clauses in $P$ does match the goal
$\mathtt{A}(x)$. Therefore the proof cannot proceed by the rule \ref{ir:lp-m}.

The same example show incompletness of the calculus of \ref{ir:lp-m},
\ref{ir:lam}, and \ref{ir:nu} in the coinductive case. The greatest Herbrand
model $\McP$ is the same and although the rule \ref{ir:nu} allows to begin the
the above proof with another step, it does not instantiate the goal
$\mathtt{A}(x)$ anyhow and therefore neither of the clauses $\kappa_1$ nor
$\kappa_2$ will be allicable in later steps. Therefore there is no way how to
construct an proof term $e$ such that $\HNF(e)$ in order to make coinductively
sound conclusion.
\end{example}

As for the completness for atomic formulate, consider the following example:

\begin{example}
    Let $\Sigma$ be signature with one predicate symbol $\mathtt{A}$ and two
    function symbols $\mathtt{f}$ and $\mathtt{g}$, the first unary and the
    other nullary.

\begin{alignat*}{3}
    \kappa_1 :~ & && \Rightarrow \mathtt{A}(\mathtt{f}(x))\\
    \kappa_2 :~ & && \Rightarrow \mathtt{A}(\mathtt{g})\\
\end{alignat*}

\noindent
The least Herbrand model $\MP = \{A(g), A(f(g)), A(f(f(g))), \dots \}$. Therefore 
$P \vDash_{ind} \mathtt{A}(x)$. However, neither the clause $\kappa_1$ nor the
clause $\kappa_2$ math $\mathtt{A}(x)$ and there is no way how to proceed with
the proof
    \begin{prooftree}
        \footnotesize
        \AxiomC{\dots}
        \RightLabel{\sc Lp-m}
        \UnaryInfC{$
            P \vdash
            e : \mathtt{A}(x)
        $}
    \end{prooftree}
\noindent
A similar argument holds in the coinductive case.

\end{example}


Take the following:

\begin{example}
    Let $P$ be the following program:

\begin{alignat*}{3}
    \kappa_1 :~ & && \mathtt{p}(\mathtt{f}(x)) \Rightarrow \mathtt{p}(x))\\
%    \kappa_2 :~ & && \Rightarrow \mathtt{A}(\mathtt{g})\\
\end{alignat*}

First, we prove $\mathtt{p}(x)$ in an extended environemnt $\Phi, \alpha_1 :
\mathtt{p}(\mathtt{a})$:

    \begin{prooftree}
        \footnotesize
        \AxiomC{}
        \RightLabel{\sc Lp-m}
        \UnaryInfC{$
            \Phi
            , (\alpha_1 : ~ \Rightarrow \mathtt{p}(\mathtt{a})) 
            , (\alpha_2 : ~ \Rightarrow \mathtt{p}(x))
            \vdash 
            \alpha : \mathtt{p}(\mathtt{f}(x))
        $}
        \RightLabel{\sc Lp-m}
        \UnaryInfC{$
            \Phi
            , (\alpha_1 : ~ \Rightarrow \mathtt{p}(\mathtt{a})) 
            , (\alpha_2 : ~ \Rightarrow \mathtt{p}(x))
            \vdash 
            \kappa_1 ~\alpha : \mathtt{p}(x)
        $}
        \RightLabel{\sc Nu'}
        \UnaryInfC{$
            \Phi
            , (\alpha_1 : ~ \Rightarrow \mathtt{p}(\mathtt{a})) 
            \vdash 
            \nu\alpha . \kappa_1 ~\alpha : \mathtt{p}(x)
        $}
    \end{prooftree}

\end{example}


==> tex/results.tex <==

\section{Soundness and Incompleteness}
\label{sec:resul}

We next prove the soundness of the corecursive resolution with respect to
greatest coinductive Herbrand model. 

\begin{theorem}
    \label{thm:sound}
    Let $F$ be a formula and let $\Phi$ be an environment.
    If $\Phi \vdash e : F$ then $\Phi \vDash F$.
\end{theorem}
\begin{proof} 
    By simultaneous induction on the structure of the proof term $e$ and the
    entailment of the formula $F$:

    Consider the case when the proof evidence $e$ has the form $\kappa$. Then in
    an environment $\Phi$ the proof evidence $e$ is entailed as
    \inference[]{}{\Phi \vdash \sigma \kappa : F}, $F$ is an atomic 
    formula and $(\kappa :~\Rightarrow F) \in \Phi$. Since $(\kappa :~\Rightarrow
    F) \in \Phi$ also $\Phi \vDash ~\Rightarrow F$ and by the Lemma
    \ref{lem:sem_prop} also $\Phi \vDash F$. Hence by the 
    Lemma~\ref{lem:inst_valid}, $\Phi \vDash \sigma F$.

    Now consider the case when $e$ has the form $\kappa~e_1,\dots,e_n$. Then in an
    environment $\Phi$, $e$ is entailed as 
    \inference[]
    {
        \Phi \vdash \sigma e_1 : B_1 \quad \cdots 
        \quad \Phi \vdash \sigma e_n : B_n  
    } 
    {
        \Phi \vdash \sigma \kappa~e_1 \cdots e_n : A
    }
    , the formula $F$ is an atomic formula such that $\sigma A = F$, for $i \in
    \{1, \dots, n\}$, $\Phi \vdash \sigma B_i$, there is a Horn formula $B_1,
    \dots, B_n \Rightarrow A$, and a judgement $(\kappa : B_1, \dots, B_n
    \Rightarrow A) \in \Phi$.  By the inductive hypothesis, for $i \in \{1,
    \dots, n\}$, $\Phi \vDash \sigma B_i$ and by the Lemma \ref{lem:sem_prop},
    $\Phi \vDash F$.
    
    Now consider the case when $e$ has the form $\alpha$. A judgement $\Phi
    \vdash \alpha : F$ is not well-formed according to the
    Definition~\ref{def:cores} and such a case is not possible.

    Now consider the case when $e$ has the form $\lambda \beta_1, \dots, \beta_n . e$.
    Then in an environment $\Phi$, $e$ is entailed as 
    \inference[]
    {
        \Phi, (\beta_1 : ~\Rightarrow B_1), \dots, (\beta_n : ~\Rightarrow B_n)
            \vdash  e : A 
    }
    {
        \Phi \vdash \lambda \beta_1,\dots,\beta_n . e : B_1,\dots,B_n
        \Rightarrow A 
    }
    , and $F$ has the form $B_1,\dots,B_n \Rightarrow A$. By the inductive
    hypothesis $\Phi, (\beta_1 : ~\Rightarrow B_1), \dots, (\beta_n :
    ~\Rightarrow B_n) \vDash A$ and by the Lemma \ref{lem:sem_prop} we obtain $\Phi
    \vDash B_1, \dots, B_n \Rightarrow A$.

    Now consider the remaining case when $e$ has the form $\nu \alpha . e$. Then
    in an environment $\Phi$, $e$ is entailed as 
    \inference[]
    {
        \Phi, (\alpha : B_1,\dots,B_n \Rightarrow A) \vdash e : B_1,\dots,B_n
            \Rightarrow A 
    } 
    {
        \Phi \vdash \nu \alpha . e : B_1,\dots,B_n \Rightarrow A 
    } 
    and $e$ is in the head normal form. Therefore $e$ has the form $\nu \alpha .
    \lambda \alpha_1, \dots, \alpha_n . \kappa~e_1 \dots e_m$ for some constant symbol
    $\kappa$. By chaining \emph{Lam} and
    \emph{Nu} rules we obtain necessarily unique sequence of resolution steps\\\\

    \inference[]
    {
        \inference[]
        {
            \Phi, (\alpha : B_1,\dots,B_n \Rightarrow A),
            (\beta_1 : ~\Rightarrow B_1), \dots, (\beta_n : ~\Rightarrow B_n)\\
            \vdash  \kappa~e_1 \dots e_m : A
        }
        {
            \Phi, (\alpha : B_1,\dots,B_n \Rightarrow A)\\
            \vdash \lambda \beta_1, \dots, \beta_n .  \kappa~e_1 \dots e_m :
            B_1,\dots,B_n \Rightarrow A 
        }
    } 
    {
        \Phi \vdash \nu \alpha .  \lambda \beta_1, \dots, \beta_n . \kappa~e_1
        \dots e_m : B_1,\dots,B_n \Rightarrow A 
    }
    ~\\
    and $A$ is entailed solely by application of the first resolution rule. By
    inspection of inductive terms $e_1$, \dots, $e_n$ either $\alpha~e'_1 \dots
    e'_n$ does not occurs among $e_1$, \dots, $e_n$ as a subterm and also $\Phi,
    (\beta_1 : ~\Rightarrow B_1), \dots, (\beta_n : ~\Rightarrow B_n) \vdash
    \kappa~e_1 \dots e_n : A$ and $\Phi \vDash B_1, \dots, B_n \Rightarrow A$ or
    there is such an ocurence. In such case there is also a resolution of $A$ by
    a term $(\kappa~e_1  \dots e_n)[\alpha~\beta_1 \dots \beta_n/\alpha~e'_1
    \dots e'_n]$ by the Lemma \ref{lem:sem_prop}.
   
    \qed
\end{proof}

Although the corecursive resolution is sound it is not complete. Firstly,
resolution is by term matching only and infinite formulae cannot be entailed:

\begin{example}
    Let $\Phi = \cdot, (\zeta : \text{nat}(\text{z})), (\sigma : \text{nat}(
    \text{s}(x)))$ and let $\text{f}^\omega$ denote the infinite term
    $\text{f}(\text{f}(\text{f}(\dots)))$. Then $\Phi \vDash 
    \text{nat}(\text{f}^\omega)$ but $\text{nat}(\text{f}^\omega)$ cannot be
    entailed as the proof evidence corresponds to the infinite proof term
    $\sigma(\sigma(\sigma(\dots)))$ since the Nu rule entails only Horn formulae
    and not atomic formulae.
\end{example}

%However, corecursive resolution is not complete even when we restrict to finite
%formulae. Inference rules as defined in the Definiton \ref{def:cores} do allow
%only certain composition of inference steps. In particular, an inference tree
%with \emph{Nu} rule in it's root is always entailed by a term in the form $\nu
%\alpha . \lambda \alpha_1, \dots, \alpha_n . \kappa~e_1 \dots e_m$ where for all
%$i$, a term $e_i$ proves an atomic formula and is resolved only by application of
%the first inference rule. Also, such resolution tree cannot be extended from the
%root since none of the inference rules accepts an evidence term in this form.
%Hence, corecursive resolution does not entail formulae, that require application
%of coinductive hypothesis on multiple places in the proof term.





